Conversational Multi-Hop Reasoning with Neural Commonsense Knowledge and Symbolic Logic Rules

One of the challenges faced by conversational agents is their inability to identify unstated presumptions of their users' commands, a task trivial for humans due to their common sense. In this paper, we propose a zero-shot commonsense reasoning system for conversational agents in an attempt to achieve this. Our reasoner uncovers unstated presumptions from user commands satisfying a general template of if-(state), then-(action), because-(goal). Our reasoner uses a state-of-the-art transformer-based generative commonsense knowledge base (KB) as its source of background knowledge for reasoning. We propose a novel and iterative knowledge query mechanism to extract multi-hop reasoning chains from the neural KB which uses symbolic logic rules to significantly reduce the search space. Similar to any KBs gathered to date, our commonsense KB is prone to missing knowledge. Therefore, we propose to conversationally elicit the missing knowledge from human users with our novel dynamic question generation strategy, which generates and presents contextualized queries to human users. We evaluate the model with a user study with human users that achieves a 35% higher success rate compared to SOTA.

==> clue_lst_dialog_fig.tex <==
\begin{figure}[h]
\begin{lstlisting}[escapechar=\%,language=corgi]
please stand by while the model loads.
command: ``If I have an early 
morning meeting then wake me up 
early because I want to be on time.''
<%\textcolor{blue-violet}{\coolname}%$> What ensures ``I am on time.''?
<%{\bf \textcolor{blue-violet}{user}}%$> [i get to work before 8]
<%\textcolor{blue-violet}{\coolname}%$> What does ``i have an early 
morning meeting'' cause that makes you 
want to ``wake up early''?
1. to be on time
2. personx is late
3. to be punctual
4. to go to work
5. to get ready
6. None of the above
Please provide number and explanation.
Due to NLP limitations, please format 
your explanation as if-then:
<%{\bf \textcolor{blue-violet}{user}}%$> [2. if I have an early morning 
meeting and i wake up at the same time 
as I usually do, then I will be late to 
my meeting.]
\end{lstlisting}
\caption{An example of \coolname's dialog interface with the user and user responses for an orange template if-then-because command. The multiple choices {\bf 1} through {\bf 5} are proofs obtained from \comet~that \coolname~is confirming with the human evaluator. The text highlighted in Blue indicates the user's responses}
\label{fig:dialog}
\end{figure}

==> logic_templates_table.tex <==
\begin{table}[t]
    \caption{Logic Templates released in \cite{corgi}. $\wedge$, $\neg$, $\coloneq$ indicate logical and, negation, and implication, respectively. $\textAction_h$ is an action that is hidden in the main utterance and $\textAction(\textState)$ indicates performing the $\textAction$ when the $\textState$ holds.}
    \label{tab:logic_templates}
\centering
\resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{lc}
        \toprule 
        \bf{Logic template} &\bf{Count} \\% \textbf{Example} & 
        \midrule
        1. \thead[l]{\blueTemplate{$(\neg(\text{\textGoal}) \coloneq \text{\textState}) \wedge$} \\ \blueTemplate{$(\text{\textGoal} \coloneq \text{\textAction}(\text{\textState}))$}} & 65 \\ % & \thead[l]{If it snows tonight \\ then wake me up early \\ because I want to arrive to work on time} & 65 \\
        % &  &\\
        2. \thead[l]{\orangeTemplate{$(\text{\textGoal} \coloneq \text{\textAction}(\text{\textState})) \wedge$} \\ \orangeTemplate{$(\neg(\text{\textGoal}) \coloneq \neg(\text{\textAction}(\text{\textState})))$}} & 50 \\ % \thead[l]{If I am walking to a meeting \\ then remind me who else is there \\ because I want to be prepared for the meeting} & 50 \\
        % & &\\
        3. \thead[l]{\greenTemplate{$(\text{\textGoal} \coloneq \text{\textAction}_h) \wedge$} \\ \greenTemplate{$(\text{\textAction}_h \coloneq \text{\textAction}(\text{\textState}))$}} & 17 \\% \thead[l]{If we are approaching Fall \\ then remind me to buy flower bulbs \\ because I want to make sure I have a pretty Spring garden.} & 17 \\
        % & &\\
        4. \thead[l]{\purpleTemplate{$(\text{\textGoal} \coloneq \text{\textState}) \wedge$} \\  \purpleTemplate{$(\neg(\text{\textGoal}) \coloneq \text{\textAction}(\text{\textState}))$}}
        & 5 \\ % \thead[l]{If I am at the grocery store but I have a trip coming up in the next week \\ then remind me not to buy perishables \\ because they will go bad while I am away} & 5 \\
        % & & \\
        % 5. \thead[l]{\pinkTemplate{$(\text{\textState} \coloneq \text{\textAction}) \wedge$} \\ \pinkTemplate{$(\text{\textAction} \coloneq \text{\textGoal})$}} & \thead[l]{If I schedule an appointment that overlaps with another appointment \\ then notify me immediately \\ because I want to notify my colleagues of the conflict.} & 1 \\
        % & & \\
        5. \redTemplate{other} & 23 \\ % \thead[l]{If tomorrow is a holiday \\ then ask me if I want to disable or change my alarms \\ because I don't want to wake up early if I don't need to go to work early.}  &23 \\
        \bottomrule
    \end{tabular}
    }
\end{table}

==> multi_hop_fig.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{images/sag_diagram.png}
\caption{Different one hop inferences between clauses}
\label{fig:onehopdiagram}
\end{figure}

==> res_multihop_all.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{images/unidirectional_HP_all.pdf}
%     \caption{Number of hops required to obtain a half-proof for the logical implication \textGoal $\coloneq$ \textAction, using unidirectional beam search. The total number of commands studied are 130.}
%     \label{fig:nhop_uni_all}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/unidirectional_HP_bar.pdf}
    \caption{Number of hops required to obtain a half-proof for the logical implication \textGoal $\coloneq$ \textAction, using unidirectional beam search. The total number of commands studied are 130. The total number of proofs at each hop is equal to 130-(number of commands proven with less number of hops)}
    \label{fig:nhop_uni_all}
\end{figure}
